Characterising the VHE diffuse emission in the central 200 parsecs of our Galaxy with H.E.S.S

The diffuse very high-energy (VHE, > 100 GeV) gamma-ray emission observed in the central 200 pc of the Milky Way by H.E.S.S. was found to follow the dense matter distribution in the Central Molecular Zone (CMZ) up to a longitudinal distance of about 130 pc to the Galactic Centre (GC), where the flux rapidly decreases. Recent sensitive H.E.S.S. analysis revealed that the cosmic-ray (CR) density profile drops with the distance to the centre, making data compatible with a steady cosmic PeVatron at the GC. In this paper, we extend this analysis to obtain for the first time a detailed characterisation of the correlation with matter and to search for additional features and individual gamma-ray sources in the inner 200 pc. Taking advantage of 250 hours of H.E.S.S. data and improved analysis techniques we perform a detailed morphology study of the diffuse VHE emission observed from the GC ridge and reconstruct its total spectrum. We show that the emission correlated with dense matter covers the full CMZ and that its flux is about half the total diffuse emission flux. We also detect some emission at higher latitude likely produced by hadronic collisions of CRs in less dense regions of the GC interstellar medium. We detect an additional emission component centred on the GC and extending over about 15 pc that is consistent with the existence of a strong CR density gradient and confirms the presence of a CR accelerator at the very centre of our Galaxy. We show that the spectrum of the full ridge diffuse emission is compatible with the one previously derived from the central regions, suggesting that a single population of particles fills the entire CMZ. Finally, we report the discovery of a VHE gamma-ray source near the GC radio arc and argue that it is produced by the pulsar wind nebula candidate G0.13-0.11.

==> authors_201610.tex <==

%% Redefine symbols for footnotes
\makeatletter
\renewcommand*{\@fnsymbol}[1]{\ifcase#1\or*\or$\dagger$\or$\ddagger$\or**\or$\dagger\dagger$\or$\ddagger\ddagger$\fi}
\makeatother

\author{\tiny H.E.S.S. Collaboration
%\and H.~Abdalla\protect\footnotemark[1] \inst{1} % main scientific contributor
\and H.~Abdalla \inst{1}
\and A.~Abramowski \inst{2}
\and F.~Aharonian \inst{3,4,5}
\and F.~Ait Benkhali \inst{3}
\and A.G.~Akhperjanian\protect\footnotemark[2] \inst{6,5} % Deceased author
\and T.~Andersson \inst{10}
\and E.O.~Ang\"uner \inst{21}
\and M.~Arakawa \inst{43}
\and M.~Arrieta \inst{15}
\and P.~Aubert \inst{24}
\and M.~Backes \inst{8}
\and A.~Balzer \inst{9}
\and M.~Barnard \inst{1}
\and Y.~Becherini \inst{10}
\and J.~Becker Tjus \inst{11}
\and D.~Berge \inst{12}
\and S.~Bernhard \inst{13}
\and K.~Bernl\"ohr \inst{3}
\and R.~Blackwell \inst{14}
\and M.~B\"ottcher \inst{1}
\and C.~Boisson \inst{15}
\and J.~Bolmont \inst{16}
\and P.~Bordas \inst{3}
\and J.~Bregeon \inst{17}
\and F.~Brun \inst{26}
\and P.~Brun \inst{18}
\and M.~Bryan \inst{9}
\and M.~B\"{u}chele \inst{36}
\and T.~Bulik \inst{19}
\and M.~Capasso \inst{29}
\and J.~Carr \inst{20}
\and S.~Casanova \inst{21,3}
\and M.~Cerruti \inst{16}
\and N.~Chakraborty \inst{3}
\and R.~Chalme-Calvet \inst{16}
\and R.C.G.~Chaves \inst{17,22}
\and A.~Chen \inst{23}
\and J.~Chevalier \inst{24}
\and M.~Chr\'etien \inst{16}
\and M.~Coffaro \inst{29}
\and S.~Colafrancesco \inst{23}
\and G.~Cologna \inst{25}
\and B.~Condon \inst{26}
\and J.~Conrad \inst{27,28}
\and Y.~Cui \inst{29}
\and I.D.~Davids \inst{1,8}
\and J.~Decock \inst{18}
\and B.~Degrange \inst{30}
\and C.~Deil \inst{3}
\and J.~Devin \inst{17}
\and P.~deWilt \inst{14}
\and L.~Dirson \inst{2}
\and A.~Djannati-Ata\"i \inst{31}
\and W.~Domainko \inst{3}
\and A.~Donath \inst{3}
\and L.O'C.~Drury \inst{4}
\and K.~Dutson \inst{33}
\and J.~Dyks \inst{34}
\and T.~Edwards \inst{3}
\and K.~Egberts \inst{35}
\and P.~Eger \inst{3}
\and J.-P.~Ernenwein \inst{20}
\and S.~Eschbach \inst{36}
\and C.~Farnier \inst{27,10}
\and S.~Fegan \inst{30}
\and M.V.~Fernandes \inst{2}
\and A.~Fiasson \inst{24}
\and G.~Fontaine \inst{30}
\and A.~F\"orster \inst{3}
\and S.~Funk \inst{36}
\and M.~F\"u{\ss}ling \inst{37}
\and S.~Gabici \inst{31}
\and M.~Gajdus \inst{7}
\and Y.A.~Gallant \inst{17}
\and T.~Garrigoux \inst{1}
\and G.~Giavitto \inst{37}
\and B.~Giebels \inst{30}
\and J.F.~Glicenstein \inst{18}
\and D.~Gottschall \inst{29}
\and A.~Goyal \inst{38}
\and M.-H.~Grondin \inst{26}
\and J.~Hahn \inst{3}
\and M.~Haupt \inst{37}
\and J.~Hawkes \inst{14}
\and G.~Heinzelmann \inst{2}
\and G.~Henri \inst{32}
\and G.~Hermann \inst{3}
\and O.~Hervet \inst{15,45}
\and J.A.~Hinton \inst{3}
\and W.~Hofmann \inst{3}
\and C.~Hoischen \inst{35}
\and M.~Holler \inst{30}
\and D.~Horns \inst{2}
\and A.~Ivascenko \inst{1}
\and H.~Iwasaki \inst{43}
\and A.~Jacholkowska \inst{16}
\and M.~Jamrozy \inst{38}
\and M.~Janiak \inst{34}
\and D.~Jankowsky \inst{36}
\and F.~Jankowsky \inst{25}
\and M.~Jingo \inst{23}
\and T.~Jogler \inst{36}
\and L.~Jouvin \inst{31}
\and I.~Jung-Richardt \inst{36}
\and M.A.~Kastendieck \inst{2}
\and K.~Katarzy{\'n}ski \inst{39}
\and M.~Katsuragawa \inst{44}
\and U.~Katz \inst{36}
\and D.~Kerszberg \inst{16}
\and D.~Khangulyan \inst{43}
\and B.~Kh\'elifi \inst{31}
\and M.~Kieffer \inst{16}
\and J.~King \inst{3}
\and S.~Klepser \inst{37}
\and D.~Klochkov \inst{29}
\and W.~Klu\'{z}niak \inst{34}
\and D.~Kolitzus \inst{13}
\and Nu.~Komin \inst{23}
\and K.~Kosack \inst{18}
\and S.~Krakau \inst{11}
\and M.~Kraus \inst{36}
\and P.P.~Kr\"uger \inst{1}
\and H.~Laffon \inst{26}
\and G.~Lamanna \inst{24}
\and J.~Lau \inst{14}
\and J.-P. Lees\inst{24}
\and J.~Lefaucheur \inst{15}
\and V.~Lefranc \inst{18}
\and A.~Lemi\`ere\protect\footnotemark[1] \inst{31}
\and M.~Lemoine-Goumard \inst{26}
\and J.-P.~Lenain \inst{16}
\and E.~Leser \inst{35}
\and T.~Lohse \inst{7}
\and M.~Lorentz \inst{18}
\and R.~Liu \inst{3}
\and R.~L\'opez-Coto \inst{3} 
\and I.~Lypova \inst{37}
\and V.~Marandon \inst{3}
\and A.~Marcowith \inst{17}
\and C.~Mariaud \inst{30}
\and R.~Marx \inst{3}
\and G.~Maurin \inst{24}
\and N.~Maxted \inst{14}
\and M.~Mayer \inst{7}
\and P.J.~Meintjes \inst{40}
\and M.~Meyer \inst{27}
\and A.M.W.~Mitchell \inst{3}
\and R.~Moderski \inst{34}
\and M.~Mohamed \inst{25}
\and L.~Mohrmann \inst{36}
\and K.~Mor{\aa} \inst{27}
\and E.~Moulin \inst{18}
\and T.~Murach \inst{7}
\and S.~Nakashima  \inst{44}
\and M.~de~Naurois \inst{30}
\and F.~Niederwanger \inst{13}
\and J.~Niemiec \inst{21}
\and L.~Oakes \inst{7}
\and P.~O'Brien \inst{33}
\and H.~Odaka \inst{44}
\and S.~\"{O}ttl \inst{13}
\and S.~Ohm \inst{37}
\and M.~Ostrowski \inst{38}
\and I.~Oya \inst{37}
\and M.~Padovani \inst{17} 
\and M.~Panter \inst{3}
\and R.D.~Parsons \inst{3}
\and N.W.~Pekeur \inst{1}
\and G.~Pelletier \inst{32}
\and C.~Perennes \inst{16}
\and P.-O.~Petrucci \inst{32}
\and B.~Peyaud \inst{18}
\and Q.~Piel \inst{24}
\and S.~Pita \inst{31}
\and H.~Poon \inst{3}
\and D.~Prokhorov \inst{10}
\and H.~Prokoph \inst{10}
\and G.~P\"uhlhofer \inst{29}
\and M.~Punch \inst{31,10}
\and A.~Quirrenbach \inst{25}
\and S.~Raab \inst{36}
\and A.~Reimer \inst{13}
\and O.~Reimer \inst{13}
\and M.~Renaud \inst{17}
\and R.~de~los~Reyes \inst{3}
\and S.~Richter \inst{1}
\and F.~Rieger \inst{3,41}
\and C.~Romoli \inst{4}
\and G.~Rowell \inst{14}
\and B.~Rudak \inst{34}
\and C.B.~Rulten \inst{15}
\and V.~Sahakian \inst{6,5}
\and S.~Saito \inst{43}
\and D.~Salek \inst{42}
\and D.A.~Sanchez \inst{24}
\and A.~Santangelo \inst{29}
\and M.~Sasaki \inst{29}
\and R.~Schlickeiser \inst{11}
\and F.~Sch\"ussler \inst{18}
\and A.~Schulz \inst{37}
\and U.~Schwanke \inst{7}
\and S.~Schwemmer \inst{25}
\and L.~Seglar-Arroyo \inst{18}
\and M.~Settimo \inst{16}
\and A.S.~Seyffert \inst{1}
\and N.~Shafi \inst{23}
\and I.~Shilon \inst{36}
\and R.~Simoni \inst{9}
\and H.~Sol \inst{15}
\and F.~Spanier \inst{1}
\and G.~Spengler \inst{27}
\and F.~Spies \inst{2}
\and {\L.}~Stawarz \inst{38}
\and R.~Steenkamp \inst{8}
\and C.~Stegmann \inst{35,37}
\and K.~Stycz \inst{37}
\and I.~Sushch \inst{1}
\and T.~Takahashi  \inst{44}
\and J.-P.~Tavernet \inst{16}
\and T.~Tavernier \inst{31}
\and A.M.~Taylor \inst{4}
\and R.~Terrier\protect\footnotemark[1] \inst{31}
\and L.~Tibaldo \inst{3}
\and D.~Tiziani \inst{36}
\and M.~Tluczykont \inst{2}
\and C.~Trichard \inst{20}
\and N.~Tsuji \inst{43}
\and R.~Tuffs \inst{3}
\and Y.~Uchiyama \inst{43}
\and D.J.~van der Walt \inst{1}
\and C.~van~Eldik \inst{36}
\and C.~van~Rensburg \inst{1} 
\and B.~van~Soelen \inst{40}
\and G.~Vasileiadis \inst{17}
\and J.~Veh \inst{36}
\and C.~Venter \inst{1}
\and A.~Viana \inst{3}
\and P.~Vincent \inst{16}
\and J.~Vink \inst{9}
\and F.~Voisin \inst{14}
\and H.J.~V\"olk \inst{3}
\and T.~Vuillaume \inst{24}
\and Z.~Wadiasingh \inst{1}
\and S.J.~Wagner \inst{25}
\and P.~Wagner \inst{7}
\and R.M.~Wagner \inst{27}
\and R.~White \inst{3}
\and A.~Wierzcholska \inst{21}
\and P.~Willmann \inst{36}
\and A.~W\"ornlein \inst{36}
\and D.~Wouters \inst{18}
\and R.~Yang \inst{3}
\and V.~Zabalza \inst{33}
\and D.~Zaborov \inst{30}
\and M.~Zacharias \inst{25}
\and R.~Zanin \inst{3}
\and A.A.~Zdziarski \inst{34}
\and A.~Zech \inst{15}
\and F.~Zefi \inst{30}
\and A.~Ziegler \inst{36}
\and N.~\.Zywucka \inst{38}
}

\institute{
Centre for Space Research, North-West University, Potchefstroom 2520, South Africa \and 
Universit\"at Hamburg, Institut f\"ur Experimentalphysik, Luruper Chaussee 149, D 22761 Hamburg, Germany \and 
Max-Planck-Institut f\"ur Kernphysik, P.O. Box 103980, D 69029 Heidelberg, Germany \and 
Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, Dublin 2, Ireland \and 
% 5
National Academy of Sciences of the Republic of Armenia,  Marshall Baghramian Avenue, 24, 0019 Yerevan, Republic of Armenia  \and
Yerevan Physics Institute, 2 Alikhanian Brothers St., 375036 Yerevan, Armenia \and
Institut f\"ur Physik, Humboldt-Universit\"at zu Berlin, Newtonstr. 15, D 12489 Berlin, Germany \and
University of Namibia, Department of Physics, Private Bag 13301, Windhoek, Namibia \and
GRAPPA, Anton Pannekoek Institute for Astronomy, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands \and
% 10
Department of Physics and Electrical Engineering, Linnaeus University,  351 95 V\"axj\"o, Sweden \and
Institut f\"ur Theoretische Physik, Lehrstuhl IV: Weltraum und Astrophysik, Ruhr-Universit\"at Bochum, D 44780 Bochum, Germany \and
GRAPPA, Anton Pannekoek Institute for Astronomy and Institute of High-Energy Physics, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands \and
Institut f\"ur Astro- und Teilchenphysik, Leopold-Franzens-Universit\"at Innsbruck, A-6020 Innsbruck, Austria \and
School of Physical Sciences, University of Adelaide, Adelaide 5005, Australia \and
% 15
LUTH, Observatoire de Paris, PSL Research University, CNRS, Universit\'e Paris Diderot, 5 Place Jules Janssen, 92190 Meudon, France \and
Sorbonne Universit\'es, UPMC Universit\'e Paris 06, Universit\'e Paris Diderot, Sorbonne Paris Cit\'e, CNRS, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), 4 place Jussieu, F-75252, Paris Cedex 5, France \and
Laboratoire Univers et Particules de Montpellier, Universit\'e Montpellier, CNRS/IN2P3,  CC 72, Place Eug\`ene Bataillon, F-34095 Montpellier Cedex 5, France \and
DSM/Irfu, CEA Saclay, F-91191 Gif-Sur-Yvette Cedex, France \and
Astronomical Observatory, The University of Warsaw, Al. Ujazdowskie 4, 00-478 Warsaw, Poland \and
% 20
Aix Marseille Universit\'e, CNRS/IN2P3, CPPM UMR 7346,  13288 Marseille, France \and
Instytut Fizyki J\c{a}drowej PAN, ul. Radzikowskiego 152, 31-342 Krak{\'o}w, Poland \and
Funded by EU FP7 Marie Curie, grant agreement No. PIEF-GA-2012-332350,  \and
School of Physics, University of the Witwatersrand, 1 Jan Smuts Avenue, Braamfontein, Johannesburg, 2050 South Africa \and
Laboratoire d'Annecy-le-Vieux de Physique des Particules, Universit\'{e} Savoie Mont-Blanc, CNRS/IN2P3, F-74941 Annecy-le-Vieux, France \and
% 25
Landessternwarte, Universit\"at Heidelberg, K\"onigstuhl, D 69117 Heidelberg, Germany \and
Universit\'e Bordeaux, CNRS/IN2P3, Centre d'\'Etudes Nucl\'eaires de Bordeaux Gradignan, 33175 Gradignan, France \and
Oskar Klein Centre, Department of Physics, Stockholm University, Albanova University Center, SE-10691 Stockholm, Sweden \and
Wallenberg Academy Fellow,  \and
Institut f\"ur Astronomie und Astrophysik, Universit\"at T\"ubingen, Sand 1, D 72076 T\"ubingen, Germany \and%29
% 30
Laboratoire Leprince-Ringuet, Ecole Polytechnique, CNRS/IN2P3, F-91128 Palaiseau, France \and
APC, AstroParticule et Cosmologie, Universit\'{e} Paris Diderot, CNRS/IN2P3, CEA/Irfu, Observatoire de Paris, Sorbonne Paris Cit\'{e}, 10, rue Alice Domon et L\'{e}onie Duquet, 75205 Paris Cedex 13, France \and
Univ. Grenoble Alpes, IPAG,  F-38000 Grenoble, France \protect\\ CNRS, IPAG, F-38000 Grenoble, France \and
Department of Physics and Astronomy, The University of Leicester, University Road, Leicester, LE1 7RH, United Kingdom \and
Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, ul. Bartycka 18, 00-716 Warsaw, Poland \and
% 35
Institut f\"ur Physik und Astronomie, Universit\"at Potsdam,  Karl-Liebknecht-Strasse 24/25, D 14476 Potsdam, Germany \and
Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, Erwin-Rommel-Str. 1, D 91058 Erlangen, Germany \and
DESY, D-15738 Zeuthen, Germany \and
Obserwatorium Astronomiczne, Uniwersytet Jagiello{\'n}ski, ul. Orla 171, 30-244 Krak{\'o}w, Poland \and
Centre for Astronomy, Faculty of Physics, Astronomy and Informatics, Nicolaus Copernicus University,  Grudziadzka 5, 87-100 Torun, Poland \and
% 40
Department of Physics, University of the Free State,  PO Box 339, Bloemfontein 9300, South Africa \and
Heisenberg Fellow (DFG), ITA Universit\"at Heidelberg, Germany  \and
GRAPPA, Institute of High-Energy Physics, University of Amsterdam,  Science Park 904, 1098 XH Amsterdam, The Netherlands \and
Department of Physics, Rikkyo University, 3-34-1 Nishi-Ikebukuro, Toshima-ku, Tokyo 171-8501, Japan \and
Japan Aerpspace Exploration Agency (JAXA), Institute of Space and Astronautical Science (ISAS), 3-1-1 Yoshinodai, Chuo-ku, Sagamihara, Kanagawa 229-8510,  Japan \and
%% Affiliation of people who left the collaboration
Now at Santa Cruz Institute for Particle Physics and Department of Physics, University of California at Santa Cruz, Santa Cruz, CA 95064, USA
}

\offprints{H.E.S.S.~collaboration,
\protect\\\email{\href{mailto:contact.hess@hess-experiment.eu}{contact.hess@hess-experiment.eu}};
\protect\\\protect\footnotemark[1] Corresponding authors
\protect\\\protect\footnotemark[2] Deceased
}




